Multi-agent Performative Prediction: From Global Stability and Optimality to Chaos

The recent framework of performative prediction is aimed at capturing settings where predictions influence the target/outcome they want to predict. In this paper, we introduce a natural multi-agent version of this framework, where multiple decision makers try to predict the same outcome. We showcase that such competition can result in interesting phenomena by proving the possibility of phase transitions from stability to instability and eventually chaos. Specifically, we present settings of multi-agent performative prediction where under sufficient conditions their dynamics lead to global stability and optimality. In the opposite direction, when the agents are not sufficiently cautious in their learning/updates rates, we show that instability and in fact formal chaos is possible. We complement our theoretical predictions with simulations showcasing the predictive power of our results.

==> name.tex <==
**1. KKT conditions**
The collection of inequalities on the partial derivatives is equivalent to the collection of KKT conditions for each player's minimization problem of decoupled performative loss.  We believe the derivation is fairly standard.  See below for more details.  

Given a collection of predictive model $\vec{\boldsymbol{\theta}}'$, agent $i$ wants to maximize its decoupled performative loss 
$L_i(\boldsymbol{\theta}^i) := \ell(\vec{\boldsymbol{\theta}}', \boldsymbol{\theta}^i)$ which is convex.  Formally,
$$\begin{aligned}
\min_{\boldsymbol{x}} \quad & L_i(\boldsymbol{x})\\
\textrm{s.t.} \quad & x_k\ge 0, \forall k\in [d]\\
  &\sum_{k\in [d]} x_k = 1\\
\end{aligned}$$
By the KKT conditions for the above convex problems, the primal $\boldsymbol{x}^*$, and dual variable $\sigma_1, \dots, \sigma_d$ and $\gamma$ satisfy
$$\begin{aligned}
    &x^*_k\ge 0, k\in[d]\\\\
    &\sum_k x^*_k = 1\\\\
    &\sigma_k\ge 0, k\in [d]\\\\
    &\sigma_k x^*_k = 0, k\in [d]\\\\
    &\frac{\partial}{\partial x_k}L_i(\boldsymbol{x}^*)-\sigma_k+\gamma = 0, k\in [d].
\end{aligned}$$
For all $l\in [d]$, by the fifth equation, $\frac{\partial}{\partial x_l}L_i(\boldsymbol{x}^*) = \sigma_l-\gamma$ which is no less than $-\gamma$ by the third equation.  Additional if $x^*_k>0$, $\sigma_k = 0$ by the fourth equation, and $\frac{\partial}{\partial x_k}L_i(\boldsymbol{x}^*) = -\gamma$.  Therefore, for all $k,l\in [d]$ with $x^*_k>0$, 
$$\frac{\partial}{\partial x_k}L_i(\boldsymbol{x}^*) \le \frac{\partial}{\partial x_l}L_i(\boldsymbol{x}^*).$$
We have shown that the optimality of $\boldsymbol{x}^*$ implies the above equation.  Conversely, if $\boldsymbol{x}^*\in \Theta$ satisfies the above equation, the KKT conditions also hold.  Therefore the above equation is an sufficient and necessary condition for maximizing agent $i$' decoupled performative loss.  

By definition of $L_i$, we have $\frac{\partial}{\partial x_k}L_i(\boldsymbol{x}^*) = \frac{\partial}{\partial x_k}\ell(\vec{\boldsymbol{\theta}}', \boldsymbol{x})|_{\boldsymbol{x} = \boldsymbol{x}^*}$.   

Therefore, $\vec{\boldsymbol{\theta}}^*$ is performative stable if and only if for all agent $i$, $\frac{\partial}{\partial x_k}\ell(\vec{\boldsymbol{\theta}}^*, \boldsymbol{x})\mid_{\boldsymbol{x} = (\vec{\boldsymbol{\theta}}^*)^i}$ which is less than $\frac{\partial}{\partial x_l}\ell(\vec{\boldsymbol{\theta}}^*, \boldsymbol{x})|_{\boldsymbol{x} = (\vec{\boldsymbol{\theta}}^*)^i}$ for all $k, l\in [d]$ with $\theta^i_k>0$.  That is 
$g^i_k(\vec{\boldsymbol{\theta}}^*)\le g^i_l(\vec{\boldsymbol{\theta}}^*)$
 for all $i\in [n]$ and $k, l\in [d]$ with $\theta^i_k>0$.  
